Learning functional sections in medical conversations: iterative pseudo-labeling and human-in-the-loop approach

Medical conversations between patients and medical professionals have implicit functional sections, such as "history taking", "summarization", "education", and "care plan." In this work, we are interested in learning to automatically extract these sections. A direct approach would require collecting large amounts of expert annotations for this task, which is inherently costly due to the contextual inter-and-intra variability between these sections. This paper presents an approach that tackles the problem of learning to classify medical dialogue into functional sections without requiring a large number of annotations. Our approach combines pseudo-labeling and human-in-the-loop. First, we bootstrap using weak supervision with pseudo-labeling to generate dialogue turn-level pseudo-labels and train a transformer-based model, which is then applied to individual sentences to create noisy sentence-level labels. Second, we iteratively refine sentence-level labels using a cluster-based human-in-the-loop approach. Each iteration requires only a few dozen annotator decisions. We evaluate the results on an expert-annotated dataset of 100 dialogues and find that while our models start with 69.5% accuracy, we can iteratively improve it to 82.5%. The code used to perform all experiments described in this paper can be found here: https://github.com/curai/curai-research/tree/main/functional-sections.

==> tables/sent-level-results.tex <==

\begin{table*}
\centering

\begin{tabular}{ccccc}
\hline
 & \multicolumn{4}{c}{\textbf{F1 score}} \\
\textbf{Class} & \textbf{Round 1} & \textbf{Round 2} & \textbf{Round 3} & \textbf{Round 4}\\
\hline
Summarization & 0.18$\pm$0.00 & 0.19$\pm$0.11 & 0.47$\pm$0.06 & \textbf{0.65}$\pm$\textbf{0.02}\\
History Taking & 0.89$\pm$0.01 & 0.9$\pm$0.00 & 0.92$\pm$0.00 & \textbf{0.93}$\pm$\textbf{0.01}\\
Education & \textbf{0.70}$\pm$\textbf{0.01} & 0.69$\pm$0.02 & 0.69$\pm$0.02 & 0.65$\pm$0.02\\ 
Care Plan & 0.55$\pm$0.02 & 0.56$\pm$0.03 & \textbf{0.57}$\pm$\textbf{0.01} & 0.55$\pm$0.02\\ 
Other & 0.90$\pm$0.00 & 0.92$\pm$0.00 & \textbf{0.93}$\pm$\textbf{0.00} & \textbf{0.93}$\pm$\textbf{0.00}\\
\Xhline{4\arrayrulewidth}
\textbf{Multi-class Accuracy*} & 69.5\%$\pm$0.00 & 74.1\%$\pm$0.00 & 80.4\%$\pm$0.01 & \textbf{82.5\%}$\pm$\textbf{0.01}\\
\hline
\multicolumn{5}{l}{* Accuracy is on the four functional classes only}\\
\end{tabular}

\caption{Sentence-level model performance: F1 scores and accuracy after each round of iterative training.  Standard deviations by retraining models with different seeds.}
\label{tab:sent-level}
\end{table*}


==> tables/turn-level-results.tex <==

\begin{table*}
\centering
\begin{tabular}{cccccc}
\hline
 & \multicolumn{5}{c}{\textbf{F1 score}} \\
\textbf{Class} & \textbf{Turn-level} & \textbf{Round 1} & \textbf{Round 2} & \textbf{Round 3} & \textbf{Round 4}\\
\hline
Summarization & 0.22$\pm$0.00 & 0.22$\pm$0.00 & 0.25$\pm$0.03 & \textbf{0.69}$\pm$\textbf{0.04} & 0.66$\pm$0.04\\
History Taking & 0.37$\pm$0.00 & 0.84$\pm$0.02 & 0.83$\pm$0.01 & 0.86$\pm$0.01 & \textbf{0.87}$\pm$\textbf{0.01}\\
Education & 0.61$\pm$0.01 & \textbf{0.77}$\pm$\textbf{0.02} & 0.69$\pm$0.05 & 0.73$\pm$0.02 & 0.65$\pm$0.04 \\ 
Care Plan & 0.31$\pm$0.04 & 0.55$\pm$0.02 & 0.55$\pm$0.03 & \textbf{0.57}$\pm$\textbf{0.01} & 0.51$\pm$0.02\\ 
Other & 0.75$\pm$0.00 & 0.89$\pm$0.01 & 0.93$\pm$0.00 & \textbf{0.95}$\pm$\textbf{0.01} & \textbf{0.95}$\pm$\textbf{0.00}\\
\Xhline{4\arrayrulewidth}
\textbf{Binary Accuracy} & 84.7\%$\pm$0.00 & \textbf{95.6}\%$\pm$0.00 & 95.2\%$\pm$0.01 & \textbf{95.6}\%$\pm$\textbf{0.00} & 94.9\%$\pm$0.00 \\
\hline
\multicolumn{6}{l}{* Accuracy is on the four functional classes only}\\
\end{tabular}

\caption{Turn-based inference improved with sentence-level model (~\S~\ref{sec:turnresults}). The column  "Turn-level" is the initial turn-level model from which sentence level model was bootstrapped. Columns Round 1--4 show the F1-score when we pool sentence-level predictions to produce turn level labels. The standard deviations are derived by retraining models with different seeds.}
\label{tab:turn-level}
\end{table*}
